Energy-Aware Adaptive Offloading of Soft Real-Time Jobs in Mobile Edge Clouds

We present a model for measuring the impact of offloading soft real-time jobs over multi-tier cloud infrastructures. The jobs originate in mobile devices and offloading strategies may choose to execute them locally, in neighbouring devices, in cloudlets or in infrastructure cloud servers. Within this specification, we put forward several such offloading strategies characterised by their differential use of the cloud tiers with the goal of optimizing execution time and/or energy consumption. We implement an instance of the model using Jay, a software framework for adaptive computation offloading in hybrid edge clouds. The framework is modular and allows the model and the offloading strategies to be seamlessly implemented while providing the tools to make informed runtime offloading decisions based on system feedback, namely through a built-in system profiler that gathers runtime information such as workload, energy consumption and available bandwidth for every participating device or server. The results show that offloading strategies sensitive to runtime conditions can effectively and dynamically adjust their offloading decisions to produce significant gains in terms of their target optimization functions, namely, execution time, energy consumption and fulfillment of job deadlines.

==> dist-new.tex <==
%           new_execution_distribution_extra
% d = 6
% LOCAL: 26.32332944832945     REMOTE: 73.67667055167055
% LOCAL: 28.456439393939394     REMOTE: 71.5435606060606
% LOCAL: 25.6155303030303     REMOTE: 74.38446969696969
% LOCAL: 62.85855588526212     REMOTE: 37.14144411473788
% LOCAL: 59.297725024728     REMOTE: 40.70227497527201
% LOCAL: 66.17210682492582     REMOTE: 33.82789317507419
% LOCAL: 48.02176063303659     REMOTE: 51.9782393669634
% LOCAL: 58.40751730959446     REMOTE: 41.59248269040554
% LOCAL: 45.796241345202766     REMOTE: 54.203758654797234
% d = 9
% LOCAL: 26.56492812742813     REMOTE: 73.43507187257188
% LOCAL: 33.54215229215229     REMOTE: 66.4578477078477
% LOCAL: 19.303613053613052     REMOTE: 80.69638694638695
% LOCAL: 81.70128585558852     REMOTE: 18.298714144411473
% LOCAL: 77.39861523244313     REMOTE: 22.601384767556876
% LOCAL: 77.54698318496538     REMOTE: 22.45301681503462
% LOCAL: 36.102868447082095     REMOTE: 63.89713155291792
% LOCAL: 59.05044510385758     REMOTE: 40.94955489614243
% LOCAL: 27.94263105835806     REMOTE: 72.05736894164194

%       new_device_execution_distribution_greys_extra
% d = 6
% 0.04826254826254826, 7.335907335907336, 25.723938223938223, 28.04054054054054, 38.851351351351354
% 0.0946969696969697, 4.8768939393939394, 29.02462121212121, 24.479166666666668, 41.52462121212121
% 0.3787878787878788, 6.534090909090909, 26.136363636363637, 25.0, 41.95075757575758
% 3.264094955489614, 14.589515331355093, 18.793273986152325, 22.799208704253214, 40.553907022749755
% 2.373887240356083, 12.215628090999012, 18.199802176063304, 26.013847675568744, 41.196834817012856
% 1.7309594460929774, 15.72700296735905, 22.35410484668645, 24.431256181998023, 35.7566765578635
% 6.726013847675569, 17.754698318496537, 22.551928783382788, 22.255192878338278, 30.712166172106826
% 4.995054401582592, 15.034619188921859, 19.782393669634025, 25.66765578635015, 34.52027695351138
% 5.835806132542038, 14.292779426310583, 16.91394658753709, 24.975272007912956, 37.982195845697326
% d = 9
% 0.04826254826254826, 12.934362934362934, 26.11003861003861, 29.198841698841697, 31.70849420849421
% 0.15060240963855423, 3.463855421686747, 25.953815261044177, 32.2289156626506, 38.20281124497992
% 0.04826254826254826, 8.88030888030888, 20.55984555984556, 21.283783783783782, 49.22779922779923
% 10.534124629080118, 17.359050445103858, 23.986152324431256, 21.810089020771514, 26.310583580613255
% 5.9347181008902075, 13.303659742828883, 19.634025717111772, 26.65677546983185, 34.47082096933729
% 6.726013847675569, 17.95252225519288, 24.975272007912956, 23.788328387734914, 26.55786350148368
% 8.852621167161226, 17.903066271018794, 23.63996043521266, 20.820969337289814, 28.783382789317507
% 5.637982195845697, 16.271018793273985, 18.694362017804153, 26.706231454005934, 32.69040553907023
% 1.4836795252225519, 14.144411473788328, 18.793273986152325, 23.590504451038576, 41.98813056379822

==> energy_table.tex <==
\begin{table*}[h!]
\caption{$\Delta$ energy table (mWh) (idle and real) with 95\% confidence interval}
  \begin{tabular}{lcccccc}
    \hline
    & Google Nexus 9 & Samsung Galaxy S7e & Samsung Galaxy Tab S5e & Xiaomi Mi 9T & Google Pixel 4\\ \hline
    Femto BALANCED (d=9) & 77.7 $\pm$ 11.0 & 416.1 $\pm$ 93.9 & 378.8 $\pm$ 50.9 & 346.9 $\pm$ 20.8 & 318.3 $\pm$ 8.3\\
    Femto TMIN (d=9) & 101.5 $\pm$ 26.8 & 173.3 $\pm$ 88.8 & 374.5 $\pm$ 58.4 & 363.2 $\pm$ 46.6 & 362.4 $\pm$ 56.7\\
    Femto HYBRID (d=9) & 61.2 $\pm$ 7.3 & 231.9 $\pm$ 93.5 & 350.6 $\pm$ 49.3 & 274.2 $\pm$ 59.2 & 441.1 $\pm$ 19.0 \\
    LF BALANCED (d=9) & 781.8 $\pm$ 238.1 & 399.7 $\pm$ 111.4 & 282.4 $\pm$ 52.9 & 279.8 $\pm$ 18.9 & 257.9 $\pm$ 29.3\\
    LF TMIN (d=9) & 652.2 $\pm$ 274.2 & 438.5 $\pm$ 82.9 & 285.9 $\pm$ 39.9 & 341.7 $\pm$ 17.5 & 256.1 $\pm$ 29.0  \\
    LF HYBRID (d=9) & 680.4 $\pm$ 243.7 & 434.8 $\pm$ 72.9 & 282.0 $\pm$ 39.0 & 287.1 $\pm$ 15.3 & 276.5 $\pm$ 33.3\\
    BALANCED (d=9) & 551.2 $\pm$ 67.9 & 416.3 $\pm$ 69.2 & 321.6 $\pm$ 73.4 & 334.2 $\pm$ 27.5 & 336.2 $\pm$ 39.6\\
    TMIN (d=9) & 484.8 $\pm$ 74.2 & 510.7 $\pm$ 179.3 & 319.7 $\pm$ 22.8 & 368.8 $\pm$ 6.7 & 337.9 $\pm$ 19.9 \\
    HYBRID (d=9) & 179.8 $\pm$ 67.5 & 460.3 $\pm$ 122.7 & 346.6 $\pm$ 65.5 & 323.7 $\pm$ 76.5 & 397.4 $\pm$ 132.3\\
    LOCAL (d=9) & 1154.9 $\pm$ 12.5 & 435.1 $\pm$ 102.1 & 255.7 $\pm$ 33.7 & 263.6 $\pm$ 4.2 & 184.6 $\pm$ 3.2 \\
    \hline\hline
    Femto BALANCED (d=6) & 75.4 $\pm$ 16.2 & 276.3 $\pm$ 65.2 & 482.3 $\pm$ 37.6 & 340.9 $\pm$ 37.0 & 356.7 $\pm$ 37.9\\
    Femto TMIN (d=6) & 85.4 $\pm$ 17.1 & 160.1 $\pm$ 66.4 & 363.4 $\pm$ 40.5 & 298.5 $\pm$ 14.3 & 390.3 $\pm$ 11.9\\
    Femto HYBRID (d=6) & 97.5 $\pm$ 31.7 & 178.8 $\pm$ 82.3 & 417.1 $\pm$ 39.6 & 303.1 $\pm$ 20.7 & 399.3 $\pm$ 21.5\\
    LF BALANCED (d=6) & 302.4 $\pm$ 26.5 & 322.1 $\pm$ 56.2 & 200.5 $\pm$ 39.5 & 294.6 $\pm$ 19.1 & 389.3 $\pm$ 13.0\\
    LF TMIN (d=6) & 279.0 $\pm$ 112.2 & 437.7 $\pm$ 68.1 & 312.4 $\pm$ 64.6 & 327.0 $\pm$ 19.0 & 356.1 $\pm$ 12.4 \\
    LF HYBRID (d=6) & 640.8 $\pm$ 172.6 & 430.6 $\pm$ 97.5 & 336.5 $\pm$ 62.6 & 315.9 $\pm$ 22.6 & 312.2 $\pm$ 31.3\\
    BALANCED (d=6) & 283.8 $\pm$ 55.4 & 411.8 $\pm$ 110.4 & 291.7 $\pm$ 57.8 & 324.9 $\pm$ 23.3 & 386.4 $\pm$ 25.2 \\
    TMIN (d=6) & 445.4 $\pm$ 87.5 & 527.0 $\pm$ 143.2 & 307.9 $\pm$ 61.4 & 352.7 $\pm$ 20.2 & 351.2 $\pm$ 31.3\\
    HYBRID (d=6) & 496.6 $\pm$ 51.9 & 476.9 $\pm$ 73.7 & 345.1 $\pm$ 34.9 & 349.9 $\pm$ 17.6 & 383.9 $\pm$ 21.5\\\hline
  \end{tabular}
\end{table*}


==> figures.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                               %%
%% Figures                       %%
%%                               %%
%% NB: this is for captions and  %%
%% Titles. All graphics must be  %%
%% submitted separately and NOT  %%
%% included in the Tex document  %%
%%                               %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
%% Do not use \listoffigures as most will included as separate files

\section*{Figures}
  \begin{figure}[h!]
  \caption{Sample figure title}
\end{figure}

\begin{figure}[h!]
  \caption{Sample figure title}
\end{figure}

==> model-saved.tex <==
\section{System Model\label{s:model}}


\begin{figure*}[h!]
\centering 
\includegraphics[width=0.8\textwidth]{images/model2.pdf}
\caption{Illustration of system model.\label{fig:model}}
\end{figure*}

\trackchange{Added subsection header for a clearer text organisation.}{
\subsection*{Overview}
}

We now put forward the system model for our adaptive offloading
framework.  

The overall rationale is as follows.  We consider a set of
hosts connected over a network, such that each host may generate
and/or execute soft real-time jobs over time.  A host may then execute
a mixture of local jobs and offloaded jobs on behalf of other hosts,
but it can also be that a host only generates or executes jobs.  In
this setting, offloading decisions can be informed and adaptive to
runtime conditions. Information broadcast amongst hosts regarding
variables such as network bandwidth and latency, host job load and
available energy provide the required feedback. 
We consider each job has a soft % estava jobs
real-time nature, meaning that it has an associated relative
deadline expressing the maximum tolerable completion time for good
QoS, and also that it requires communication among hosts in the case
of offloading to supply job inputs (before the job's computation can
proceed) and obtain job outputs (when the computation is done).

\trackchange{}{
In what follows, we first lay out the base model 
concerning job characteristics and the time and energy costs
for offloading, and then present sample offloading strategies over that model.
} 

\trackchange{Added subsection header for a clearer text organisation.}{
\subsection*{Base definitions}
}

We associate each job~$j$ with a release time~$r(j)$, a termination
time~$t(j) > r(j)$, a relative deadline~$d(j)$, an originating
host~$\hL$ from a set of hosts~$\Hosts$, and, finally, a computation
host~$\hE$ also in~$\Hosts$.  When~$j$ is clear in context, these
properties are simply denoted respectively as~$r$,~$t$,~$d$, ~$\hL$,
and~$\hE$.  We say that the deadline of the job is fulfilled
if~$t \le r + d$.  Furthermore, we say the job executes locally
at~$\hL$ when~$\hL = \hE$, and that it is offloaded from~$\hL$
to~$\hE$ when~$\hL \neq \hE$.

In the scenario of runtime adaptive offloading, for job~$j$ and at
time~$r$, an offloading decision is made at time~$r$ to
determine~$\hE$. We assume that decision to be computed locally (at
$\hL$) and to have negligible overhead.  In the case of offloading
($\hL \neq \hE$), we assume that network communication needs to take
place between~$\hL$ and~$\hE$ for the inputs of~$j$ (data but possibly
also code) to be available at~$\hE$ before~$j$ starts, and, later,
once the computation~$j$ terminates, for the outputs to be transmitted
back from~$\hE$ to $\hL$.  This is illustrated in
Figure~\ref{fig:model}, along with the formulation for time and energy
overheads during offloading.


We consider the offloading decision to be informed by estimates of
completion time and energy consumption as follows.  Per each
host~$h \in \Hosts$ (including $\hL$) we model the estimated
completion time and energy consumption of a given job $j$, $\ttime(h)$ and $\ener(h)$,
respectively as:
$$
\ttime(h) = \TI(h) + \TC(h) + \TO(h)
$$
$$
\ener(h) = \EI(h) + \EC(h) + \EO(h)
$$
where time ($\ttime$) and energy ($\ener$) are factored into a sum of
three terms: $\TI$, $\EI$: the (time and energy) costs of input
offloading job~$j$; $\TC$, $\EC$: the (time and energy) costs of the
actual computation for job~$j$, and; $\TO$, $\EO$: the (time and
energy) costs of downloading outputs of job~$j$. Note that, given that
there is no need for network communication when~$h = \hL$, we should
necessarily have $\TI(\hL) = \EI(\hL) = \TO(\hL) = \EO(\hL) = 0$.

Regarding energy, our aim is not merely to account for the energy
consumption at the originating host ($\hL$) of a job, but also in the
computation host in the case of offloading ($\hE$).  This means first that
network I/O expressed by the~$\EI$ and~$\EO$ should account for
the energy consumption both in~$\hL$ and~$\hE$: sending inputs
from~$\hL$ to~$\hE$ requires energy to be consumed by $\hL$ in
uploading the inputs, and~$\hE$ to download, and vice-versa in the
case of outputs. Since~$\EI$ and~$\EO$ are respectively dependent on the transmission
times~$\TI$ and $\TO$ and the power consumption when doing so, we
model $\EI$ and $\EO$ as follows: 
$$
\EI(h) = \TI(h) \times \PI(h)
$$
$$
\EO(h) = \TO(h) \times \PO(h)
$$
where~$\PI$ and~$\PO$ are estimates for the power consumed per time unit
at both~$\hL$ and $\hE$\footnote{in these formulae, when clear from the context, the index of $h$ is
  omitted for the sake of simplicity}, 
when, respectively, sending job inputs from~$\hL$ to~$\hE$ and 
receiving job outputs at~$\hL$ from~$\hE$.

Moreover, the $\EC$ term reflects the cost of executing the job
remotely at~$\hE$, but, as illustrated in Figure~\ref{fig:model}, it
should only account for an estimate of the energy consumption
\emph{while}~$\hE$ is effectively performing the computation for
job~$j$ for an amount of time~$\TE$, rather than the energy
consumption over the total period~$\TC$, during which the job may at
times be pending (e.g., waiting for other jobs in $\hE$ to
complete). Thus, we write:
$$
\EC(h) = \TE(h) \times \PC(h)
$$
where~$\PC$ is an estimate for the power consumed per time unit at~$h$
due to the execution of the actual computation of~$j$ at~$h$.

\trackchange{Added subsection header for a clearer text organisation.}{
\subsection*{Offloading strategies}
}


\begin{figure*}[h!]
\centering 
\includegraphics[width=0.8\textwidth]{images/offloading-strategies.pdf}
\caption{Illustration of offloading strategies.\label{fig:strategies}}
\end{figure*}

We can now express offloading strategies that may account (or not) for
completion time and energy consumption.
We do so for the cases of
interest instantiated within \Jay{} and covered in our evaluation later
in the paper. 
\trackchange{New figure added.}{
We use Figure~\ref{fig:strategies} as an illustration for the main rationale
in the offloading strategies. The figure illustrates the offloading decision
for a job originating at host $\hL=h_0$ in an environment with four other hosts, 
$h_1$ to $h_4$, such that each host may have different values 
regarding the estimates for time and energy consumption ($\ttime$ and $\ener$).
}

The simplest case is that of no offloading, which we
designate as the {\rm LOCAL} strategy
\trackchange{}{
(i.e., as illustrated in Figure~\ref{fig:strategies} jobs always execute locally).
}:
$$
{\rm LOCAL} \quad \equiv \quad \hE = \hL
$$
The choice may also be fixed to a special host $\hS \neq \hL$
(assuming $\hS$ does not generate jobs), for instance a cloud server
that is responsible for executing all jobs 
\trackchange{}{
(in Figure~\ref{fig:strategies}, $\hS$ is host $h_1$)}
, designated as the {\rm SERVER} strategy:
$$
{\rm SERVER} \quad \equiv \quad \hE = \hS
$$
%{

\trackchange{}{
In the case illustrated by Figure~\ref{fig:strategies} that {\rm LOCAL}
and {\rm SERVER} would not lead to optimal choices regarding time and/or energy, as
there are hosts that can execute the job faster than $\hL$ and $\hS$ ($h_2$ and $h_4$),
or that may consume less energy to do so ($h_3$ and $h_4$).
}
Adaptiveness comes into play if we account for the $\ttime$ and/or
$\ener$ estimates. 

 A strategy that seeks to minimize the completion
time of job, but ignoring energy consumption, can be defined as:
$$
{\rm TMIN} \quad \equiv \quad \hE = {\rm argmin}_{h \:\in\: \Hosts} \: \ttime(h)
$$
\trackchange{}{
Hence, in Figure~\ref{fig:strategies} we have $\hE = h_2$ for {\rm TMIN}.
}
In analogous manner, a strategy that seeks to minimize energy
consumption can be defined as:
$$
{\rm EMIN} \quad \equiv \quad \hE = {\rm argmin}_{h \:\in\: \Hosts} \: \ener(h)
$$ % TODO explain better
but it will not however attend to QoS requirements in terms of
deadline fulfilment, i.e., $\hE$ may be chosen regardless of whether
$\ttime(h_E) \le d$ or not. 
\trackchange{}{
This is illustrated in Figure~\ref{fig:strategies}, where $\hE = h_3$
for {\rm TMIN} but $T(h_3) > d$.
}
Additionally, the most energy-efficient
hosts will tend to be preferred. These hosts may possibly become
congested with too many jobs whose execution can therefore be much
delayed in time.  The above strategy can be refined meaningfully to
counter for these problems as:
$$
{\rm HYBRID} \quad \equiv \quad \hE = {\rm argmin}_{h \:\in\: \Hosts \::\: \ttime(h) \le d} \: \ener(h)
$$
balancing both time and energy costs and the fulfilment of $d$, as it
expresses that $\hE$ is chosen as the host which consumes less energy
amongst those that can satisfy the job deadline
($h \:\in\: \Hosts \::\: \ttime(h) \le d$). 
\trackchange{}{
This is illustrated in Figure~\ref{fig:strategies}, where $\hE = h_4$ is
the host with lower $\ener$ value, among those with a $\ttime$ value lower than $d$
(all except $h_3$).
}
 In the case where {\rm
  HYBRID} yields no result, i.e., no host is estimated to be able to
satisfy the job deadline, the offloading decision may for instance
fallback to {\rm TMIN} trying to complete the job as fast as possible
anyway or to simply cancel the job altogether.

% TODO: new
\trackchange{Extended discussion}{

The  {\rm TMIN} and {\rm HYBRID} strategies may  lead to an imbalance between host loads, 
in the sense that most time-efficient and/or energy-efficient hosts will tend to have higher loads. This
may be counter-productive if the hosts are stake are battery-constrained and we wish for instance
to extend battery lifetime of all hosts more evenly, as in~\cite{TODO}.
To spread the load more evenly, a balanced selection scheme of hosts amongst those
that can comply with a job deadline can be defined. For instance, a
balanced selection policy can be defined as:
$$
{\rm BALANCED} \quad \equiv \quad \hE = {\rm random} \:\{ h \:\in\: \Hosts \::\: \ttime(h) \le d \:\}
$$
i.e., $\hE$ is randomly selected among the hosts that can comply with the deadline.
In this case, the offloading choice may not be energy-optimal or time-optimal, but the random
choice will tend to promote a more balanced distribution of jobs. We could also refine ${\rm BALANCED}$ 
to be explicitly energy-aware by refining the definition with constraints for energy consumption or battery level thresholds in addition to the job's deadline. Also, in alternative, a round-robin job distribution could be considered
instead to enforce stricter load balancing.

Finally, we put in perspective the following trait found in a number of systems, e.g.~\cite{TODO}:
restricted offloading where a job is only offloaded 
if the local host~$\hL$ is judged to be incapable of fulfilling the job's QoS, 
usually seeking costs due to network transmission, e.g., in terms of energy, amount of data, billing costs.
 % TODO refs
In correspondence, 
we can formulate a ``local-first'' strategy ${\rm LF}_f$, where~$f$ is the policy
to apply in the case of offloading, as:
$$
{\rm LF} [f] \quad \equiv \quad \hE = \left\{
\begin{array}{@{}rl@{}}
\hL, & \mbox{ if } \ttime(\hL) \le d \bigstrut \\
f, & \mbox{otherwise}
\end{array}
\right.
$$
i.e., a job executes locally if the completion time estimate complies
with deadline, otherwise~$f$ is evaluated to decide where the job should run, e.g.,
we can define the ${\rm LF}[{\rm TMIN}]$, ${\rm LF}[{\rm HYBRID}]$, or ${\rm LF}[{\rm BALANCED}]$
strategies.
%The ${\rm LF}_f$ formulation also illustrates that the general approach of our model can flexibly accommodate for
%the composition of offloading strategies and compose them. 

}





==> rwork-backup.tex <==
\section*{Related work}\label{s:rwork}

Many systems have been proposed to leverage the power of nearby devices to increase
computation capacity of a single mobile device. Cloudlets, introduced by Satyanarayanan et al.~\cite{Satyanarayanan2009}~\cite{Satyanarayanan2012}~\cite{Satyanarayanan2013}~\cite{Satyanarayanan2015a}, were amongst the first approaches for computational perfomance improvements
by offloading computations from a less capable mobile device to a dedicated workstation
on the viccinity of the network with higher computational power. Multiple mobile device
cooperation, forming an Edge-Cloud, models were also developed~\cite{hyraxmsc} to try and divide heavy workloads for a single mobile device across a group of devices, that although limited
in performance, with cooperation, can perform heavy tasks.

More recently, several similar approaches for Edge-Computing have been published. Such as
Fog computing~\cite{Bonomi2012}~\cite{Yousefpour2017} (or Mist Computing~\cite{Liyanage2016}) which is an highly virtualized platform that provides compute, storage and networking services between end devices and traditional cloud computing data centers located at the edge of network. Cyber Foraging~\cite{Balan2002} (first applied to mobile devices in~\cite{Verbelen2012}) uses opportunistically discovered servers in the environment to improve the performance of interactive applications and distributed file systems on mobile clients.
Volunteer computing~\cite{Anderson2004}~\cite{Ryden2014}~\cite{Anderson2019}~\cite{Alonso-Monsalve2018}~\cite{Marosi2013}~\cite{Funai2014} is a platform where users donate their
computing power to a larger cause. This concept has been around since the early 2000's when users shared their computer power and has been evolving towards mobile phones. Nowadays,
users can share contribute to a larger project simply by installing an application on their device.
Femto Clouds~\cite{Habak2015} are systems which provide a dynamic, self-configuring and multi-device mobile cloud out of a cluster of mobile devices. These systems are usually coordinated by a selected device (the coordinator) and are resillient to churn.
Drop Computing~\cite{Ciobanu2019} which is yet another definition of an edge computing system, proposes the concept of decentralized computing over multilayered networks, combining
cloud and wireless technologies over a social crowd formed between mobile and edge devices.

Several systems such as Hyrax~\cite{hyraxmsc}, mCrowd~\cite{Yan2009}, CDroid~\cite{Barbera2013}, COSMOS~\cite{Shi2014}, POMAC~\cite{Hassan2014}, MVR~\cite{Wei2017}, Cumulus~\cite{Gedawy2017}, ActorEdge~\cite{Aske2017}, HERMES~\cite{Kao2017}. Rodrigues et. al.~\cite{Rodrigues2018}~\cite{rodrigues2019middleware}, Aura~\cite{Hasan2018}, Circa~\cite{Lin2020}, Oregano~\cite{Teofilo2017}~\cite{Sanches2020}, Jay~\cite{fmec20_jay} focus on increasing mobile device capabilites by offloading computations to other devices in
viccinity or to more powerful cloudlets and clouds or by serving as cache servers improving overall QoS of end-users.

% Data-Centric Distributed Computing on Networks of Mobile Devices~\cite{Sanches2020}

% Volunteer Computing:
% Towards a volunteer cloud system~\cite{Marosi2013}
% Nebula: Distributed edge cloud for data intensive computing~\cite{Ryden2014}
% Extending volunteer computing through mobile ad hoc networking~\cite{Funai2014}
% A heterogeneous mobile cloud computing model for hybrid clouds~\cite{Alonso-Monsalve2018}
% BOINC: A Platform for Volunteer Computing~cite{Anderson2019}

% Drop Computing:
% Drop computing: Ad-hoc dynamic collaborative computing~\cite{Ciobanu2019}

% Cyber Foraging:
% AIOLOS: Middleware for improving mobile application performance through cyber foraging~\cite{Verbelen2012}

% Fog Computing:
% Fog Computing: Towards Minimizing Delay in the Internet of Things~\cite{Yousefpour2017}
% MePaaS: Mobile-embedded platform as a service for distributing fog computing to edge nodes~\cite{Liyanage2016}
% Fog computing and its role in the internet of things~\cite{Bonomi2012}


%FALTA POR
% Green Computing ~\cite{Jain2013}
% Using Wi-Fi to save energy via p2p remote execution ~\cite{Kristensen2010a}
% Tradeoff between performance improvement and energy saving in mobile cloud offloading systems ~\cite{Wu2013}

While all of those systems address computation distribution amongst groups of devices,
energy concerns mobile devices have been a problem since early mobile devices emerged~\cite{Satyanarayanan1997}~\cite{Flinn1999a}~\cite{Flinn1999}~\cite{Flinn2000}~\cite{Flinn2002}~\cite{Flinn2004}~\cite{Satyanarayanan2005}~\cite{Gurun2006}, and since the end of 2000s, these concerns have been tackled by several systems for smartphones in specific.

MAUI~\cite{Cuervoy2010} was one of the first frameworks to try and improve smartphone Batteries
via code offload. In this work, the authors explore the problem severity of battery duration for smartphones while performing computationally intensive tasks. In
the framework developed, programmers can annotate methods that can be executed on a cloud server. MAUI instruments each method, using their profiler to make smart decisions
on wether it would be benefitial to offload a method or not. If a disconnection occurs, the method is executed locally. MAUI works on .NET Common Language Runtime (CLR) applications.
Energy monitoring in MAUI was done by using a hardware power meter attached to the mobile device battery. To map cpu consumption to battery consumption they collected cpu
utilization samples and the corresponding energy consumption, building a simple linear model for power consumption using least-squares linear regression. The authors verified
good improvements in energy consumption and performance using their framework with a close-by server.

AIOLOS~\cite{Verbelen2012} is a cyber foraging middleware framework for Android. AIOLOS uses an estimation model that takes into account server resources and network state
to device at runtime whether or not a method call should be offloaded. AIOLOS focus on two objectives: optimize energy and optimize execution time. In order to select
which chunks of code should be candidates to be offloaded, programmers have to annotate their selected classes and follow a set of rules set in place by the middleware.

CloneCloud~\cite{Chun2011} uses a different approach from MAUI in the sense that it performs an offline static and dynamic analysis of the application, creating code
partitions that will be runt either locally or offloaded. This decision is made during code partitioning and tries to minimize a cost function. For energy consumption
estimations they use 3 variables (CPU, Screen On and network state) mapping them to a power value. This system runs on Android with modified Dalvik VM modifications by
the authors and Android-x86 VMs that run on the server. As in MAUI, authors show that for certaint applications they can improve greatly the energy consumption
and execution time.

In Cuckoo~\cite{Kemp2012} the authors developed a service that, at runtime,  intercepts all method call and makes a decision wether to offload or not a method. In the version presented the decision was to allways offload methods with only wether the remote resource is reacheable or not as context information. Cuckoo server allows for multiple clients that discover this resource via sharing of QR codes.

Synergy~\cite{Kharbanda2012} is a framework that allows tasks to be distributed amongst a group of devices (discovered using Alljoyn). In order to save energy,
this framework performs frequency and voltage scaling to reduce devices cpu frequencies and voltage when running a task distributed across a group of devices.
In order for an application to take any advantage of this framework it must be parallelizable, since portions are distributed in the network.

ThinkAir~\cite{Kosta2012} exploits the concept of smartphone virtualization on the cloud and provides method-level computation offloading. In ThinkAir
developers have to anotate offloadable methods and compile theirs application using the auther own customized NDK and code generator. This framework
has four offloading policies: Execution Time, Energy, Execution Time and Energy, and Execution Time, Energy and Cost. The cost optimization factors
the cost of renting and using a cloud server. Energy estimations is based on PowerTutor~\cite{yang2012powertutor} and it uses power consumption of individual
elements of a smartphone (e.g. GPS, Screen, CPU, etc) and sums them to make an estimation.

Phone2Cloud~\cite{Xia2014} is a computation offloading-based system for energy and performance improvements on smartphones by offloading computations to
the cloud. This system is composed of seven components, including a bandwidth monitor, a resource monitor and an execution time predictor. The offloading
decision decides wether to offload the whole or a part of an application to a cloud based on offloading-decision making algorithm that can be customized.
In order to make energy estimations on the smartphone they use cpu power consumption and multiply it with expected application time. To estimate
energy spent on the mobile phone if a computation is offloaded to the cloud they account in energy of sending and receiving data and the power
consumption of waiting for computation to finish. If the tradeoff of offloading versus executing locally is benefitial, they offload the application.


% In~\cite{Bahwaireth2016} present a collection of efficient techniques for energy optimization in Mobile Cloud Computing .... . In~\cite{Mao2016} [Dynamic Computation Offloading for Mobile-Edge Computing with Energy Harvesting Devices] . In~\cite{Liu2016} [Multi-device task offloading with time-constraints for energy efficiency in mobile cloud computing] ... . ~\cite{Jalali2016} [Fog computing may help to save energy in cloud computing] ... . ~\cite{Zhao2016} [Energy-efficient task offloading for multiuser mobile cloud computing] ... . ~\cite{Chen2017} [Exploiting Massive D2D Collaboration for Energy-Efficient Mobile Edge Computing] ... . In ~\cite{Gedawy2018} and ~\cite{Gedawy2018a} Gedawy et. al. [An energy-aware iot femtocloud system][Awakening the Cloud Within: Energy-Aware Task Scheduling on Edge IoT Devices] ... . In~\cite{Guo2019} ... . In~\cite{Wu2020} ... .


ULOOF~\cite{Neto2018} is a computation offload framework for Android apps (APK). This framework
offloads computations on a method level, using pre-processed apks with anotated
offloadable methods. This pre-processing generates a prepared APK with modified
code to provide the offloading logic. The system is designed to offload computations to cloudlet or cloud machines
that run Android-X86~\cite{huang2011android} VMs with a specific server applications that has an
execution environment similar to a smartphone Android version (Dalvik or ART).
The authors tested ULOOF using simulation and on a small testbed of real devices
energy consumption, but the authors did not notice a large advantage of offloading
to a cloudlet instead of a cloud. To test the framework, the authors implemented
two applications that were not very data intensive, but that were computationally
intensive and irregular. They also noticed that their estimations were much more accurate in terms of energy
consumption on remote devices than locally, this is due to most of the energy
spent on each method was on data transfers and not on the computation itself.
The overhead of each method offloading decision was less than 40ms and for
short execution methods, the overhead reached at most 32\% of the execution time,
which corresponded to 33ms. The average execution time was 513.47ms.
For future work, the authors pretend to estimate the mobility of user to improve
predictions and address multiple users for a single server scenarios.

Honeybee~\cite{Fernando2013}~\cite{Fernando2019} is a mobile edge computing system that supports
P2P work sharing among dynamic mobile nodes. Honeybee API, a programming framework for developing mobile crowd computing applications
focus on the dynamism of mobile edge networks, implementing a work stealing algorithm for load balancing and multiple
fault-tolerance and recovery strategies. While their main focus is computation speedup, they also verify that offloading
computations had an impact on the task delegator, reducing its energy consumption when there were multiple workers in
the network.

RAMOS~\cite{Gedawy2020} is a Femto Cloud platform that schedules tasks according to two different metrics -
energy efficiency and latency minimization. This platform was written in Java for the controller
node, Android for Android smartphones and Java fot IOT devices (Raspberry pi's and Intel Edison).
The system consists of a controller that has several modules, such as a task originator interface,
task manager scheduler and task characteristics estimator. In the controller there's also a worker
manager and an accuracy enhancing module. Each worker has a resounce monitor, hearbeats manager, energy profiler
and a tasks manager. Each mobile/IOT device has a limited \textit{energy budget}, is connected to a controller
and has a FIFO task queue, from which only one task is executed at a given time.
In order to test the performance of the system, authors used a desktop machine as a controller
and a set of iot and android devices as worker nodes. They assign an energy budget to each worker
and emulate an energy model with fixed consumptions per data megabyte, and megaflop (transfer and
execution energy costs). They gather results comparing the RAMOS platform with two naive schedulers: first come first server
and round robin. They analyse the scheduler results according to the Relative Completion Time,
Relative Device Utilization, Computation Throughtput and Total Energy Consumption.
The results show that the system can improve up to 40\% time speedup on time latency minimization and up to 30\%
energy efficiency when compared to the naive schedulers.

\begin{table}
\caption{Comparing~\Jay{} with Related Work}
\label{tab:rw_compare}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{0.09\textwidth} p{0.09\textwidth} p{0.09\textwidth} p{0.09\textwidth} p{0.09\textwidth} p{0.09\textwidth} p{0.09\textwidth} p{0.09\textwidth} p{0.09\textwidth} p{0.09\textwidth} p{0.09\textwidth}}
\toprule
Name & Objective & Code Modifications & Granularity & External Coordination? & Devices Supported & Built-in Energy-Aware? & Load Balanced? & Modular? & Dynamic connections? & Extensible?\\
\midrule
~\Jay{} & Minimize latency. Minimize energy. Custom objectives & Submit tasks~\Jay{} & Job & No & Android, x86 (JVM) & Yes, dynamic at runtime & Yes, Scheduler Specific & Yes & Yes & Yes \\
ULOOF & Energy efficiency. Latency minimization & Method anotations. Pre-processed APK & Method & No & Android, Android-x86 & Static energy curve per device & Yes & No & Yes & No\\
RAMOS & Energy efficiency. Latency minimization & Built around controller & Task & Yes &  Android (\& IOT), x86 for Controller (Java) & Static budget per device & Yes & No & Yes & No \\
Honeybee & Performance gain. Energy conservation & Submit tasks to delegator & Task & No & Android & No (\%) & Yes, work stealing & No & Yes & No\\
MAUI & Energy conservation. & Method anotations & Method & No & .NET CLR & Static Linear curve & No & No & No & No\\
CloneCloud & Performance gain. Energy conservation & Off-line Partitioning & Code Partitions & No & Android w\ mod. Dalvik, Android-x86 & Static Curve & No & No & No & No\\
Synergy & Energy conservation & Parallelizable applications & Task & No & Android, Linux/ Windows & No/Energy Budget & Yes & No & Yes & No\\
ThinkAir & Performance gain. Energy conservation. Cost Reduction & Method annotations. Pre-processed & Method & No & Android, Android-VMs & Yes. PowerTutor & No & No & No & No\\
Phone2Cloud & Energy conservation & Application & Application & No & Android & Yes & No & No & No & No\\
% COSMOS & \\
% POMAC & \\
% MVR & \\
% Aura & \\
% Hermes & \\
\bottomrule
\end{tabular}%
}
\end{table}


% \begin{figure}
% \includegraphics[width=\columnwidth]{images/esquema_tabela_rw.png}
% \caption{ESQUEMA DE TABELA PARA COMPARAR SISTEMAS}
% \label{fig:EXEMPLO_TABELA}
% \end{figure}


% Finally, in ~\cite{Amsel2010}~\cite{Goel2012}~\cite{Corral2013}~\cite{Jagroep2015}~\cite{Jagroep2016} tools and techniques are described to estimate power consumptions via software.... .


==> tables.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                               %%
%% Tables                        %%
%%                               %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Use of \listoftables is discouraged.
%%
\section*{Tables}
\begin{table}[h!]
\caption{Sample table title. This is where the description of the table should go}
  \begin{tabular}{cccc}
    \hline
    & B1  &B2   & B3\\ \hline
    A1 & 0.1 & 0.2 & 0.3\\
    A2 & ... & ..  & .\\
    A3 & ..  & .   & .\\ \hline
  \end{tabular}
\end{table}

